Integrating connection search in graph queries

Graph data management and querying has many practical applications. When graphs are very heterogeneous and/or users are unfamiliar with their structure, they may need to find how two or more groups of nodes are connected in a graph, even when users are not able to describe the connections. This is only partially supported by existing query languages, which allow searching for paths, but not for trees connecting three or more node groups. The latter is related to the NP-hard Group Steiner Tree problem, and has been previously considered for keyword search in databases. In this work, we formally show how to integrate connecting tree patterns (CTPs, in short) within a graph query language such as SPARQL or Cypher, leading to an Extended Query Language (or EQL, in short). We then study a set of algorithms for evaluating CTPs; we generalize prior keyword search work, most importantly by (i) considering bidirectional edge traversal and (ii) allowing users to select any score function for ranking CTP results. To cope with very large search spaces, we propose an efficient pruning technique and formally establish a large set of cases where our algorithm, MOLESP, is complete even with pruning. Our experiments validate the performance of our CTP and EQL evaluation algorithms on a large set of synthetic and real-world workloads.

==> conclusions.tex <==
\section{Conclusions}\label{conclusion}
In this paper, we have proposed the syntax and semantics of a novel query language that supports combining the structured elements in a query with unstructured fragments. Additionally, we provided an efficient query processing algorithm for evaluating such queries. In particular, we provide an efficient and scalable implementation for processing the computationally expensive CTP queries. Our evaluations and comparisons with the state-of-the-art graph databases and query systems demonstrate the expressiveness and efficiency of our system.
As part of our future work, we would like to optimize the execution order of the CTP and BGP queries based on their dependencies and cost estimations. Additionally, we would also like to optimise the CTPs further to be multithreaded and reuse prior computations. Another interesting extension of our work is to design the language and implement provision for temporal CTPs, that is, enabling specifications and querying for temporal connections.

==> preliminaries.tex <==
\section{Preliminaries}\label{prelims}




